Overlapping Schwarz methods with GenEO coarse spaces for indefinite and non-self-adjoint problems

GenEO (`Generalised Eigenvalue problems on the Overlap') is a method for computing an operator-dependent spectral coarse space to be combined with local solves on subdomains to form a robust parallel domain decomposition preconditioner for elliptic PDEs. It has previously been proved, in the self-adjoint and positive-definite case, that this method, when used as a preconditioner for conjugate gradients, yields iteration numbers which are completely independent of the heterogeneity of the coefficient field of the partial differential operator. We extend this theory to the case of convection-diffusion-reaction problems, which may be non-self-adjoint and indefinite, and whose discretisations are solved with preconditioned GMRES. The GenEO coarse space is defined here using a generalised eigenvalue problem based on a self-adjoint and positive-definite subproblem. We prove estimates on GMRES iteration counts which are independent of the variation of the coefficient of the diffusion term in the operator and depend only very mildly on variations of the other coefficients. These are proved under the assumption that the subdomain diameter is sufficiently small and the eigenvalue tolerance for building the coarse space is sufficiently large. While the iteration number estimates do grow as the non-self-adjointness and indefiniteness of the operator increases, practical tests indicate the deterioration is much milder. Thus we obtain an iterative solver which is efficient in parallel and very effective for a wide range of convection--diffusion--reaction problems.

==> introduction.tex <==
%!TEX root = ./indefinite_geneo.tex
\section{Introduction}\label{sec-1}

This paper is concerned with the theory and implementation of two-level domain decomposition preconditioners for finite element  systems arising from indefinite and/or non-self-adjoint elliptic boundary value problems with rough or highly variable coefficients.  We analyse and test a method which is scalable with respect to the number of subdomains and also robust to  heterogeneity, backed up by supporting theory. The method is developed for the following
scalar second-order (convection--diffusion--reaction) PDE with homogeneous Dirichlet boundary conditions:
\begin{subequations}
\label{eq:2-1}
\begin{align}
-\mathrm{div}( A \nabla u) + \mathbf{b}\cdot\nabla u + cu &= f & & \text{in } \Omega, \\
u &= 0 & & \text{on } \partial\Omega,
\end{align}
\end{subequations}
posed on a bounded  polygonal or Lipschitz  polyhedral domain $\Omega\subset \mathbb{R}^{d}$ ($d=2,3$). As well as a weak regularity assumption on the
coefficients $A, \mathbf{b}$ and $c$ (Assumption \ref{ass:1}), we will assume that
\eqref{eq:2-1}  has a unique weak solution $u\in H^1(\Omega)$ for all $f \in L^2(\Omega)$.


In overlapping domain  decomposition methods, the global domain $\Omega$ is covered by a set of
overlapping subdomains~$\Omega_i$, $i=1,\ldots N$,  and the  classical one-level additive Schwarz preconditioner
is built from partial solutions on each subdomain. Since this preconditioner is not in general scalable as the number of subdomains grows,  an  additional global  coarse solve  is usually  added to enhance scalability, as well as  robustness
with respect to coefficient heterogeneity.

\bigskip

\noindent {\bf Aim of the paper and related literature.}
The construction of suitable coarse spaces has enjoyed intensive recent  interest. Since classical
coarse spaces (piecewise polynomials on a coarse grid, e.g., \cite{cai,toselli}) are not
robust for highly heterogeneous problems,
a number of groups have developed operator-dependent coarse spaces
which are better adapted to the heterogeneity, an early example being \cite{ivanrob}.
Most recently,  attention has focussed on
`spectral' coarse spaces  which are built from selected modes of local generalised eigenvalue problems.
The first proposals of this technique for domain decomposition preconditioning  were \cite{galvis1,galvis2}.  The use of local spectral information is important in   the related but different context of robust approximation techniques
for multiscale PDE problems, e.g., \cite{babuska,efendiev,ma1,ma2}.

This paper focuses on the GenEO coarse space, first proposed in
\cite{spillane:2014} for    general coercive, self-adjoint systems of PDEs (e.g., \eqref{eq:2-1}
with $\mathbf{b} =0$ and $c \geq 0$).   In \cite{spillane:2014},  it was
rigorously proved that (when combined with a one-level method and using  preconditioned conjugate gradients as the iterative solver), the resulting algorithm enjoys not only
scalability with respect to  the number of subdomains, but also robustness with respect to coefficient variation.     Recent contributions in this very active field  include \cite{giraud, klawonn,peter} and \cite{spillane:2021}, while  more  complete lists of contributions can be found in the literature surveys in, e.g.,  \cite{spillane:2014} and \cite{galvis:2018:ODD}.

While all the methods cited so far were developed for SPD problems,  where the behaviour of the  local
eigenspaces  can be more readily  analysed, there has also been considerable (so far mostly empirical)  progress on applying related techniques to non-coercive problems. Most of this has been for
the Helmholtz problem at high frequency, although \cite{nataf:2021} contains recent work on saddle-point systems.
For Helmholtz, the first publications include \cite{conen:2014,bootland:2021:OTD}, while recent work in
\cite{bootland:2021:ACS} compares the performance of several spectral coarse spaces
for high-frequency Helmholtz problems in a high performance environment. One of the most encouraging coarse spaces for Helmholtz problems
(called `H-GenEO' in \cite{bootland:2021:ACS,bootland:2021:GCS}) has  promising robustness properties at high frequency, but, since it  involves solving for local generalised eigenvalues of the Helmholtz operator,
it is beyond the reach of the present theory. However, the fact that
H-GenEO behaves similarly to the method analysed in this paper at lower frequencies, see \cite{bootland:2021:GCS}, motivated the current work.

Our other primary motivation was  to find out how well the  GenEO technology works (both in theory and in practice) for general  non-self-adjoint and indefinite PDEs of the form \eqref{eq:2-1}.
The GenEO coarse space that we analyse here is the same as the space
previously proposed and analysed in the SPD case. Thus our numerical results here indicate  the results which  can be expected when any standard GenEO code
is used for the more general problem \eqref{eq:2-1}.
The main contribution of the present paper therefore is the analysis of how GenEO
performs as a preconditioner for GMRES when applied to \eqref{eq:2-1}
and, in particular, its  dependence  on heterogeneity, indefiniteness, and lack of self-adjointness.

Since the FE systems that arise from \eqref{eq:2-1} are  in general non-Hermitian,
we use  GMRES as the iterative solver
and our main tool for convergence  analysis is the  `Elman theory'
(\cite{elman} or \cite[Lemma C.11]{toselli}), which requires   an upper bound for the norm of
the preconditioned matrix and a lower  bound on the distance of its field of values from the origin.
The number of GMRES iterates to achieve a given error tolerance is then a function of these two bounds.
Thus, the dependence  of these bounds on the parameters of the problem (e.g., mesh size, subdomain
size, overlap, heterogeneity, and strength of indefiniteness/non-self-adjointness) is of paramount
interest when analysing the robustness and scalability of the preconditioner.
The use of the Elman theory  in domain decomposition goes back to Cai and Widlund  \cite{cai} (see also \cite[Section 11]{toselli}), who used
classical linear piecewise polynomials on a coarse grid
without attention to coefficient heterogeneity.
Analogous  results for Maxwell's equations were obtained in \cite{pasciak}.

\bigskip

\noindent {\bf The main results of this paper.}  Our main theoretical result, Theorem~\ref{thm:2-1}, provides rigorous upper bounds on the coarse mesh
diameter $H$ and on the `eigenvalue tolerance'~$\Theta$ (for the local GenEO eigenproblems) which ensure
that GMRES enjoys robust and mesh-independent convergence  when applied to the preconditioned problem.
Reducing   $H$  and $\Theta$ still  further would  improve  GMRES convergence  but increase  cost:
smaller     $\Theta$ means that more  local eigenfunctions are incorporated into the coarse space;
smaller  $H$ means that more
local eigenvalue problems have to be solved, although the size of the local subdomains becomes smaller and, in practice,  fewer eigenfunctions are needed on each subdomain. Optimal choices of $\Theta$ and $H$  are typically determined empirically.
Since Theorem \ref{thm:2-1}  is quite technical, by way of introduction we present here
the result when it is specialised to the following simpler, yet instructive,   example.

\begin{example}[An indefinite but self-adjoint problem]   \label{ex:1} \em
Consider problem \eqref{eq:2-1} with $\mathbf{b} = \mathbf{0}$, and $c(x) = - \kappa$ where $\kappa$ is a positive constant. That is
\begin{align}
-{\rm div}( A \nabla u) -  \kappa u = f,
\label{DP}
\end{align}
with homogeneous Dirichlet boundary conditions.  Let  $a_{\min}$ and $a_{\max}$ be, respectively, lower and upper spectral bounds on $A$ (see \eqref{eq:Abound}). Without loss of generality,  we assume that $a_{\min} = 1$ and that the diameter $D_\Omega$ of $\Omega$ satisfies $D_\Omega \le 1$. (Otherwise the problem can be rescaled to achieve these requirements.) The GenEO coarse space is based on the $m_i$ (dominant) eigenfunctions corresponding to the smallest eigenvalues $\lambda^i_1,\ldots,\lambda_{m_i}^i$ of the generalised eigenvalue problem   on  $\Omega_i $  defined in \eqref{eq:2-18}.  To obtain a robust rate of convergence for GMRES that depends only on $k_0$ (the maximum  number of times any point is overlapped by the subdomains $\Omega_i$), Theorem \ref{thm:2-1} proves that
the following conditions on the `eigenvalue tolerance' $\Theta := 1/\min_{i=1}^N  \lambda^i_{m_i+1} $ and on the  (coarse) mesh diameter $H$ are sufficient:
\begin{align} \label{eq:bdLam0}
H \ \lesssim \ \kappa^{-1} \quad \text{and} \quad  \Theta^{1/2} \lesssim (\Cstab^* + 1)^{-1} \,  \kappa^{-2}.
\end{align}
Here   $\Cstab^*>0$ is the stability constant for the adjoint problem to \eqref{eq:2-1} and is
defined in \eqref{eq:Cstabstar}. It blows up as  the distance of $\kappa$ from an eigenvalue of the Dirichlet problem for $-{\rm div} (A \nabla u)$ decreases.
The hidden constants in \eqref{eq:bdLam0}  are independent of the fine mesh size $h$, as well as $a_{\max}$,  $\kappa$, and $\Cstab^*$, but can depend on  $k_0$.
Thus, under  conditions \eqref{eq:bdLam0} the rate of convergence of GMRES depends only on $k_0$.
For constant $A$, the first  condition in \eqref{eq:bdLam0} is exactly the one required to ensure that the piecewise linear finite element discretization of \eqref{eq:2-1} on a coarse mesh of diameter $H$ is uniquely solvable (see, e.g., \cite{cai}).
\end{example}

The full statement of Theorem \ref{thm:2-1}  for a spatially- and sign-varying $c$ and for a nonzero, spatially varying  convection coefficient  $\mathbf{b}$ is structurally  similar. Sufficient conditions for robustness are obtained by replacing   $\kappa^{-1}$ and $\kappa^{-2}$  in the two bounds  \eqref{eq:bdLam0}, respectively, by
$$(1 +  \|\mathbf{b}\|_{\infty} + \|c\|_{\infty}  )^{-1},  $$
and
$$(1+  \|\mathbf{b}\|_{\infty}  + \|c\|_{\infty}  )^{-1}(1+ \|\mathbf{b}\|_{\infty} + \|\nabla \cdot \mathbf{b}\|_{\infty} + \|c\|_{\infty} )^{-1}.$$
By making a small change to the GenEO construction,  the contribution from $c$ in  these bounds can be removed if $c$ is uniformly non-negative. We remark also that our results do not depend on the spatial variation of $A$  or $c$ and depend on the variation of $\mathbf{b}$ only through its divergence.

The proof of Theorem \ref{thm:2-1} is obtained by estimating the norm and the field of values of the preconditioned problem in the energy inner product induced by the second order operator in \eqref{eq:2-1},  and then applying the Elman estimate. Several technical difficulties have to be overcome, particularly:  (i) since the regularity assumptions on the coefficients $A$, $\mathbf{b}$, and $c$ are minimal, there is no a priori regularity for solutions of \eqref{eq:2-1} beyond $H^1$; (ii) because of the indefiniteness and non-self-adjointness of \eqref{eq:2-1}, the existence and stability of solutions of both local and coarse space subproblems
has to be established,  and this is the first source of conditions on $H$ and $\Theta$; (iii) all estimates should be explicit in the coefficients $A$, $\mathbf{b}$, and $c$, and as sharp as possible.

After the proof of  Theorem \ref{thm:2-1}, we remark  that restricting the result to the special case $\mathbf{b} = \mathbf{0}$ and $c = 0$, we obtain essentially the same result as in \cite{spillane:2014}, which is interesting because the latter makes use of `self-adjoint' technology, working with eigenvalue and condition number estimates and does not estimate the field of values as is required in \cite{elman}.
%\iggnote{Chupeng: Please leave this ednote in to remind me to add this at the end of Theorem \ref{thm:2-1}}

In Section \ref{sec:numerical} we give substantial numerical experiments illustrating the theory. All experiments are on rectangular domains with uniform fine meshes.  Highlights of these results include: (i) for  problem \eqref{eq:2-1},  with $A = I$,  $\mathbf{b} = 0$, and $c = -\kappa$ constant,  the standard GenEO preconditioner is remarkably effective even up to about $\kappa = 1000$; (ii) in the case $A = I$, $c = 0$, and $\mathbf{b}$ variable, the method is effective up to about $\Vert \mathbf{b} \Vert_\infty = 1000$, with the results only degrading moderately as the divergence of
$\mathbf{b}$ increases from zero; (iii) the results above  hardly change when $A = I$ is changed to a highly heterogeneous field; (iv) provided the ratio of  overlap width to subdomain diameter is held fixed as $h\rightarrow 0$, the dimension of the GenEO coarse space is independent of $h$; (v) the method provides a
very effective preconditioner for systems arising from implicit time-stepping applied to convection--diffusion--reaction problems, and the preconditioner can be assembled once and used for all choices of (variable) time-steps.

We remark that, while Theorem \ref{thm:2-1} provides convergence estimates for  `weighted'  GMRES
applied  in the `energy' inner product, our numerical experiments use  standard GMRES and the    Euclidean inner product. In Corollary \ref{cor:Euclidean}
we show that standard GMRES attains the same accuracy as weighted GMRES after
a few extra iterations which grow only logarithmically in $h^{-1}$ and in the contrast of the matrix $A$.
The empirical observation that weighted and standard GMRES yield similar iteration counts in domain decomposition methods has been made before, e.g., \cite{cai_zou,ivan} and a result related but not identical to Corollary \ref{cor:Euclidean} is given in \cite[Corollary 5.8]{shihua}.

In our experiments the rather stringent looking condition on the eigenvalue tolerance in \eqref{eq:bdLam0} appears to be overly pessimistic and the coarse space sizes necessary to achieve full robustness in practice
are moderate. Similar observations were made in \cite{cai}, for homogeneous but indefinite problems and classical coarse spaces.

\bigskip

\noindent {\bf Plan of the paper.} In Section \ref{prob} we give some background to domain decomposition for
\eqref{eq:2-1} and introduce the GenEO preconditioner. In Section \ref{sec-2} we prove some of the
central technical estimates  concerning solutions of the subproblems, which are then used in Section \ref{Proof} to prove the main theorem. Finally, numerical experiments are detailed in Section \ref{sec:numerical}.

==> numerical_results.tex <==
%!TEX root = ./indefinite_geneo.tex
\section{Numerical experiments}
\label{sec:numerical}

In this section we provide numerical results primarily for the two model problems: Firstly, an indefinite elliptic problem (where $\kappa > 0$)
\begin{subequations}
\label{eq:helmholtz}
\begin{align}
-\mathrm{div}( A \nabla u) - \kappa u &= f & & \text{in } \Omega, \\
u &= 0 & & \text{on } \partial\Omega,
\end{align}
where the splitting in \eqref{eq:splitc} used is given by
\begin{align}
\label{eq:helmholtz-splitting}
c^+ =0 \quad \text{and} \quad  c^- = - \kappa.
\end{align}
\end{subequations}
Secondly, a convection--diffusion problem
\begin{subequations}
\label{eq:convdiff}
\begin{align}
-\mathrm{div}( A \nabla u) + \mathbf{b}\cdot\nabla u &= f & & \text{in } \Omega, \\
u &= 0 & & \text{on } \partial\Omega,
\end{align}
where the splitting in \eqref{eq:splitc} used is given by
\begin{align}
\label{eq:convdiff-splitting}
c^+ = 0 = c^-.
\end{align}
\end{subequations}
Unless stated otherwise, in all our computations $\Omega = (0,1)^2$.

We first detail the common numerical setup. Our computations are performed using FreeFem \cite{hecht:2012} (\url{http://freefem.org/}), in particular within the \texttt{ffddm} framework. We perform experiments in 2D and discretise on uniform square grids with mesh spacing $h$, triangulating along one set of diagonals to form P1 elements. As the right-hand side $f$ we impose a point source at the centre of the domain $\Omega$.

To precondition the large sparse linear systems that arise from
discretisation, unless otherwise stated, we utilise a two-level additive Schwarz preconditioner
where the GenEO coarse space is incorporated additively, as in
\eqref{eq:2-24}. This is used within a right-preconditioned GMRES
iteration, which is terminated once a relative reduction of the
residual of at least $10^{-6}$ has been achieved, or otherwise after a
maximum of 1000 iterations (denoted in the tables below by `$1000+$').
%(In this case we mark the run with $\times$ to
%indicate the lack of sufficient convergence.)
For the local subdomains
we use a uniform decomposition into $N$ square subdomains which,
unless stated otherwise, are then extended by adding only the
fine-mesh elements which touch them (yielding a `minimal overlap'
scenario). Within the GenEO coarse space we take all eigenvectors
corresponding to eigenvalues satisfying the eigenvalue threshold
$\lambda < \lambda_\text{max}$. Unless otherwise stated, we use the
threshold parameter $\lambda_\text{max} = 0.5$ which, in light of
Definition \ref{def:2-2}, ensures that $\Theta \le 2$ in our
numerical experiments. Note that this means we do not make $\Theta$
particularly small in practice, although it is necessary in
theory. To solve the local generalised eigenvalue problems we use
ARPACK \cite{arpack:1998}, as interfaced through FreeFem.

\subsection{The case of homogeneous diffusion coefficient}
\label{subsec:numerics-homogeneous}

To illustrate some of the basic properties of the GenEO method, we first consider some simple homogeneous
test cases (i.e., with $A = I$), exploring how  indefiniteness/non-self-adjointness  affects performance.
In Table~\ref{Table:Indefinite_homogeneous_nglob600} we display results for problem \eqref{eq:helmholtz}, varying the strength of the indefiniteness through increasing $\kappa$. We see that the GenEO coarse space, built only from the positive
(Laplacian) part of the problem (recall \eqref{eq:helmholtz-splitting}), works surprisingly well  and provides a scalable solver for $\kappa \leq 1000$.
However, once $\kappa$ is too large the performance degrades and for
$\kappa = 10000$ the method lacks robustness and scalability, the
underlying problem now being highly indefinite.

\begin{table}[t]
	\centering
	\tabulinesep=1.2mm
	\begin{tabu}{c|ccccc}
		& \multicolumn{5}{c}{$N$} \\
		$\kappa$ & 4  & 16  & 36  & 64  & 100 \\
		\hline
		1 & 16  & 17 & 17 & 18 & 18 \\
		10 & 17  & 18 & 18 & 18 & 18 \\
		100 & 24  & 27 & 26 & 23 & 23 \\
		1000 & 40  & 98 & 102 & 113 & 89 \\
		10000 & 144  & 431 & 660 & $\!\!1000+\!\!$ & $\!\!1000+\!\!$
	\end{tabu}
	% \begin{tabu}{c|ccccccccc}
	% 	& \multicolumn{9}{c}{$N$} \\
	% 	$\kappa$ & 4 & 9 & 16 & 25 & 36 & 49 & 64 & 81 & 100 \\
	% 	\hline
	% 	1 & 16 & 17 & 17 & 17 & 17 & 18 & 18 & 18 & 18 \\
	% 	10 & 17 & 17 & 18 & 18 & 18 & 18 & 18 & 19 & 18 \\
	% 	100 & 24 & 26 & 27 & 26 & 26 & 24 & 23 & 24 & 23 \\
	% 	1000 & 40 & 75 & 98 & 110 & 102 & 118 & 113 & 126 & 89 \\
	% 	10000 & 144 & 269 & 431 & 515 & 660 & 755 & $\times$ & $\times$ & $\times$
	% \end{tabu}
	\caption{Iteration counts for the homogeneous, elliptic, indefinite problem \eqref{eq:helmholtz}, varying the parameter $\kappa$ and the number of subdomains $N$ for fixed $h = 1/600$.}
	\label{Table:Indefinite_homogeneous_nglob600}
\end{table}

Turning now to non-self-adjointness, Table~\ref{Table:Convection_zero_div_homogeneous_nglob600} (left) gives results for \eqref{eq:convdiff} with $A = I$ and
\begin{align}
\label{conv:zero-div}
\mathbf{b} = b \, (1+\sin(2\pi(2y-x))) (2,1)^{T},
\end{align}
The non-self-adjointness can be increased by varying $b$.
In this case, $\nabla \cdot \mathbf{b} = 0$ and so in
\eqref{eq:constants} $C_2(\mathbf{b},
c^-) = C_1(\mathbf{b}, c^-)$, thus improving
the estimate in Theorem \ref{thm:2-1}. We observe that, also in this case,
the GenEO coarse space works well and provides
a scalable method for $b$ up to at least $1000$. For $b = 10000$
the convection term appears too strong and the iteration counts
deteriorate.

\begin{table}[t]
	\centering
	\tabulinesep=1.2mm
	\begin{tabu}{c|ccccc}
		& \multicolumn{5}{c}{$N$} \\
		$b$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		1 & 18 & 18 & 18 & 18 & 18 \\
		10 & 28 & 26 & 23 & 22 & 21 \\
		100 & 35 & 34 & 30 & 28 & 27 \\
		1000 & 57 & 59 & 63 & 62 & 59 \\
		10000 & 172 & 276 & 355 & 472 & 512
	\end{tabu} \qquad\qquad
	% \begin{tabu}{c|ccccccccc}
	% 	& \multicolumn{9}{c}{$N$} \\
	% 	$b$ & 4 & 9 & 16 & 25 & 36 & 49 & 64 & 81 & 100 \\
	% 	\hline
	% 	1 & 18 & 17 & 18 & 17 & 18 & 18 & 18 & 18 & 18 \\
	% 	10 & 28 & 26 & 26 & 24 & 23 & 23 & 22 & 22 & 21 \\
	% 	100 & 35 & 37 & 34 & 31 & 30 & 28 & 28 & 27 & 27 \\
	% 	1000 & 57 & 62 & 59 & 61 & 63 & 58 & 62 & 57 & 59 \\
	% 	10000 & 172 & 224 & 276 & 315 & 355 & 367 & 472 & 439 & 512
	% \end{tabu}
	\begin{tabu}{c|ccccc}
		& \multicolumn{5}{c}{$N$} \\
		$b$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		1 & 18 & 18 & 18 & 18 & 18 \\
		10 & 28 & 26 & 23 & 22 & 21 \\
		100 & 39 & 43 & 35 & 29 & 25 \\
		1000 & 72 & 107 & 71 & 74 & 63 \\
		10000 & 201 & 450 & 708 & 835 & 837
	\end{tabu}
	% \begin{tabu}{c|ccccccccc}
	% 	& \multicolumn{9}{c}{$N$} \\
	% 	$b$ & 4 & 9 & 16 & 25 & 36 & 49 & 64 & 81 & 100 \\
	% 	\hline
	% 	1 & 18 & 17 & 18 & 17 & 18 & 18 & 18 & 18 & 18 \\
	% 	10 & 28 & 28 & 26 & 24 & 23 & 22 & 22 & 21 & 21 \\
	% 	100 & 39 & 43 & 43 & 35 & 35 & 29 & 29 & 26 & 25 \\
	% 	1000 & 72 & 105 & 107 & 89 & 71 & 79 & 74 & 73 & 63 \\
	% 	10000 & 201 & 352 & 450 & 603 & 708 & 795 & 835 & 866 & 837
	% \end{tabu}
\caption{Iteration counts for the convection--diffusion
          problem \eqref{eq:convdiff}, with homogeneous diffusion $A = I$ and
          convection coefficient \eqref{conv:zero-div} with zero
          divergence (left) and \eqref{conv:non-zero-div} with
          nonzero divergence (right), varying the constant $b$ and
        the number of subdomains $N$ for fixed $h = 1/600$.}
	\label{Table:Convection_zero_div_homogeneous_nglob600}
\end{table}

We also consider problem  \eqref{eq:convdiff} with a convection
field with non-vanishing divergence, namely
\begin{align}
\label{conv:non-zero-div}
\mathbf{b} = b \, (1+\sin(2\pi(2x+y))) (2,1)^{T}.
\end{align}
These results are given in Table
\ref{Table:Convection_zero_div_homogeneous_nglob600} (right) and
are similar to those in the left table,
displaying robustness except in the most convection-dominated case.
However, for higher $b$ the iteration counts become larger compared to the zero-divergence case,
illustrating that the strength of  $\nabla \cdot \mathbf{b}$ does play a role, as
predicted by the theory through the constant $C_2$ (given in
\eqref{eq:constants}). We consider the impact of the convection field
further in Section \ref{subsec:numerics-convfield}.

% \begin{table}[ht]
% 	\centering
% 	\caption{Iteration counts for the homogeneous convection--diffusion problem with non-zero-divergence convection coefficient \eqref{conv:non-zero-div}, varying the parameter $b$ and the number of subdomains $N$, with a fixed $h = 1/600$.}
% %	\caption{Results for the homogeneous convection--diffusion problem with non-zero-divergence convection coefficient $\mathbf{b} = b \, (1+\sin(2\pi(2x+y))) (2,1)^{T}$, varying the parameter $b$ (which controls the size of the asymmetry) and the number of subdomains $N$, with a fixed $h = 1/600$.}
% 	\label{Table:Convection_non-zero_div_homogeneous_nglob600}
% 	\tabulinesep=1.2mm
% 	\footnotesize
% 	\begin{tabu}{c|ccccccccc}
% 		& \multicolumn{9}{c}{$N$} \\
% 		$b$ & 4 & 9 & 16 & 25 & 36 & 49 & 64 & 81 & 100 \\
% 		\hline
% 		1 & 18 & 17 & 18 & 17 & 18 & 18 & 18 & 18 & 18 \\
% 		10 & 28 & 28 & 26 & 24 & 23 & 22 & 22 & 21 & 21 \\
% 		100 & 39 & 43 & 43 & 35 & 35 & 29 & 29 & 26 & 25 \\
% 		1000 & 72 & 105 & 107 & 89 & 71 & 79 & 74 & 73 & 63 \\
% 		10000 & 201 & 352 & 450 & 603 & 708 & 795 & 835 & 866 & 837
% 	\end{tabu}
% \end{table}

\subsection{The case of a heterogeneous diffusion coefficient}
\label{subsec:numerics-heterogeneous}

\begin{figure}[t]
	\centering
	\begin{tikzpicture}[scale=0.6]
		\foreach \x in {0,2,4,6,8}
		\foreach \y in {0,2,4,6,8}
		\fill[gray,opacity=((\y+1)*0.1)] (\x,\y) -- (\x+1,\y) -- (\x+1,\y+1) -- (\x,\y+1) -- cycle;
		\fill[gray,opacity=1] (9*0.16,9*0.63) -- (9*0.16,9*0.68) -- (9*0.72,9*0.47) -- (9*0.72,9*0.42) -- cycle;
		\fill[white,opacity=1] (9*0.22,9*0.03) -- (9*0.22,9*0.11) -- (9*0.94,9*0.23) -- (9*0.94,9*0.15) -- cycle;
		\fill[gray,opacity=0.5] (9*0.22,9*0.03) -- (9*0.22,9*0.11) -- (9*0.94,9*0.23) -- (9*0.94,9*0.15) -- cycle;
		\draw (0,0) -- (9,0) -- (9,9) -- (0,9) -- cycle;
	\end{tikzpicture}
	\caption{The heterogeneous function $a(\mathbf{x})$ within the inclusions and channels test problem. The shading gives the value of $a(\mathbf{x})$ with the darkest shade being $a(\mathbf{x}) = a_\text{max}$, where $a_\text{max}>1$ is a parameter, and the background white taking the value $a(\mathbf{x}) = 1$.}
	\label{Fig:InclusionsAndChannels}
\end{figure}
We now consider the same experiments as in the previous subsection but with the diffusion coefficient $A$ being heterogeneous. In particular, we will consider an ``inclusions and channels'' problem, akin to that in \cite{nataf:2011}. Here, the heterogeneous coefficient is given by
\begin{align}
A(\mathbf{x}) = a(\mathbf{x}) I, \quad \text{where }
a(\mathbf{x}) \text{ is given in Figure~\ref{Fig:InclusionsAndChannels}}. \label{eq:hetcoeff}
\end{align}
The function $a(\mathbf{x})$ represents a number of inclusions, whose contrast
with the background value of $a_\text{min} = 1$ varies depending
on the $y$-coordinate, along with two channels which run across the
inclusions and link through a larger part of the domain, one with
$a(\mathbf{x}) = a_\text{max}$ and one with $a(\mathbf{x}) =
\frac{1}{2} a_\text{max}$. This represents a challenging heterogeneous
problem for iterative solvers even in the self-adjoint and
positive-definite case (i.e., $\mathbf{b} = 0$ or $\kappa = 0$).
The strength of the heterogeneity is determined by the contrast parameter $a_\text{max}$.

Results for problem \eqref{eq:helmholtz} are given in Table~\ref{Table:Heterogeneous_nglob600} (left)
while results for problem \eqref{eq:convdiff} with zero-divergence
$\mathbf{b}$ are in Table~\ref{Table:Heterogeneous_nglob600}
(right). Results for the case when $\nabla \cdot \mathbf{b} \not=0$ are
similar to those in the zero-divergence case,  and thus
omitted. We see that in all cases where the GenEO coarse space led
to a robust method for the homogeneous problem, it does also for the
heterogeneous problem and, moreover, is robust to the strength of
the heterogeneity (here determined by $a_\text{max}$). In the highly
indefinite or highly non-self-adjoint cases, where the method
struggles already for homogeneous problems, the lower iteration
counts for some of the heterogeneous problems may stem from the fact
that in some parts of the domain the heterogeneity in fact reduces
the strength of the indefiniteness or of the convection term
locally.  For instance, consider the part $\Omega'$ of the domain
where $a$ is constant and has the largest value $a_\text{max}$
(indicated by the darkest shade in Figure
\ref{Fig:InclusionsAndChannels}). Then, restricting
\eqref{eq:helmholtz} to $\Omega'$, we see  that effectively \eqref{eq:helmholtz} reduces to
\begin{align*}
-\Delta u - \left(a_\text{max}^{-1}\kappa\right) u = a_\text{max}^{-1} f,
\end{align*}
hence reducing the effective indefiniteness in this region when $a_\text{max} > 1$ is large.
\begin{table}[t]
	\centering
	\tabulinesep=1.2mm
	\begin{tabu}{cc|ccccc}
		\multicolumn{2}{c|}{} & \multicolumn{5}{c}{$N$} \\
		$\kappa$ & $a_\text{max}$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		1 & 5  & 18 & 18 & 18 & 18 & 18   \\
		1 & 10 & 18 & 18 & 18 & 18 & 19   \\
%		1 & 20 & 18 & 18 & 19 & 19 & 19  \\
		1 & 50 & 18 & 18 & 19 & 19 & 19   \\
		\hline
		10 & 5  & 18 & 18 & 18 & 19 & 19   \\
		10 & 10 & 18 & 18 & 19 & 19 & 19   \\
%		10 & 20 & 18 & 18 & 19 & 19 & 19   \\
		10 & 50 & 18 & 18 & 20 & 19 & 19   \\
		\hline
		100 & 5  & 27 & 30 & 26 & 23 & 22   \\
		100 & 10 & 26 & 26 & 24 & 23 & 22   \\
%		100 & 20 & 26 & 24 & 23 & 22 & 21   \\
		100 & 50 & 23 & 22 & 22 & 20 & 20   \\
		\hline
		1000 & 5  & 70 & 140 & 177 & 167 & 138   \\
		1000 & 10 & 58 & 118 & 146 & 131 & 108   \\
%		1000 & 20 & 59 & 107 & 131 & 123 & 109   \\
		1000 & 50 & 48 & 94  & 114 & 106 & 99    \\
		\hline
		10000 & 5  & 193 & 524 & 906 & $\!\!1000+\!\!$ & $\!\!1000+\!\!$  \\
		10000 & 10 & 162 & 457 & 815 & $\!\!1000+\!\!$& $\!\!1000+\!\!$ \\
%		10000 & 20 & 146 & 398 & 776 & $\times$ & $\times$   \\
		10000 & 50 & 114 & 318 & 704 & 888      & $\!\!1000+\!\!$
	\end{tabu}\quad
	\begin{tabu}{cc|ccccc}
		\multicolumn{2}{c|}{} & \multicolumn{5}{c}{$N$} \\
		 $b$ & $a_\text{max}$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		 1 & 5  & 18 & 18 & 18 & 18 & 18 \\
		 1 & 10 & 18 & 18 & 19 & 19 & 19 \\
%		 1 & 20 & 18 & 18 & 19 & 19 & 19 \\
		 1 & 50 & 18 & 18 & 19 & 19 & 19 \\
		\hline
		10 & 5  & 25 & 25 & 23 & 22 & 21 \\
		10 & 10 & 24 & 24 & 23 & 21 & 20 \\
%		10 & 20 & 23 & 24 & 23 & 21 & 20 \\
		10 & 50 & 23 & 23 & 23 & 21 & 21 \\
		\hline
		100 & 5  & 39 & 36 & 31 & 28 & 27 \\
		100 & 10 & 38 & 36 & 31 & 27 & 26 \\
%		100 & 20 & 36 & 36 & 30 & 27 & 26 \\
		100 & 50 & 32 & 34 & 29 & 27 & 26 \\
		\hline
		1000 & 5  & 51 & 59 & 57 & 57 & 54 \\
		1000 & 10 & 49 & 53 & 54 & 56 & 53 \\
%		1000 & 20 & 50 & 54 & 54 & 55 & 51 \\
		1000 & 50 & 53 & 57 & 55 & 54 & 51 \\
		\hline
		10000 & 5  & 142 & 232 & 298 & 370 & 408 \\
		10000 & 10 & 121 & 180 & 261 & 320 & 328 \\
%		10000 & 20 & 101 & 158 & 236 & 284 & 300 \\
		10000 & 50 & 87  & 148 & 224 & 261 & 278
	\end{tabu}
% 	\begin{tabu}{cc|ccccc||cc|ccccc}
% 		\multicolumn{2}{c|}{} & \multicolumn{5}{c||}{$N$} \\
% 		$\kappa$ & $a_\text{max}$ & 4 & 16 & 36 & 64 & 100 & $b$ & $a_\text{max}$ & 4 & 16 & 36 & 64 & 100 \\
% 		\hline
% 		1 & 5  & 18 & 18 & 18 & 18 & 18   & 1 & 5  & 18 & 18 & 18 & 18 & 18 \\
% 		1 & 10 & 18 & 18 & 18 & 18 & 19   & 1 & 10 & 18 & 18 & 19 & 19 & 19 \\
% %		1 & 20 & 18 & 18 & 19 & 19 & 19   & 1 & 20 & 18 & 18 & 19 & 19 & 19 \\
% 		1 & 50 & 18 & 18 & 19 & 19 & 19   & 1 & 50 & 18 & 18 & 19 & 19 & 19 \\
% 		\hline
% 		10 & 5  & 18 & 18 & 18 & 19 & 19   & 10 & 5  & 25 & 25 & 23 & 22 & 21 \\
% 		10 & 10 & 18 & 18 & 19 & 19 & 19   & 10 & 10 & 24 & 24 & 23 & 21 & 20 \\
% %		10 & 20 & 18 & 18 & 19 & 19 & 19   & 10 & 20 & 23 & 24 & 23 & 21 & 20 \\
% 		10 & 50 & 18 & 18 & 20 & 19 & 19   & 10 & 50 & 23 & 23 & 23 & 21 & 21 \\
% 		\hline
% 		100 & 5  & 27 & 30 & 26 & 23 & 22   & 100 & 5  & 39 & 36 & 31 & 28 & 27 \\
% 		100 & 10 & 26 & 26 & 24 & 23 & 22   & 100 & 10 & 38 & 36 & 31 & 27 & 26 \\
% %		100 & 20 & 26 & 24 & 23 & 22 & 21   & 100 & 20 & 36 & 36 & 30 & 27 & 26 \\
% 		100 & 50 & 23 & 22 & 22 & 20 & 20   & 100 & 50 & 32 & 34 & 29 & 27 & 26 \\
% 		\hline
% 		1000 & 5  & 70 & 140 & 177 & 167 & 138   & 1000 & 5  & 51 & 59 & 57 & 57 & 54 \\
% 		1000 & 10 & 58 & 118 & 146 & 131 & 108   & 1000 & 10 & 49 & 53 & 54 & 56 & 53 \\
% %		1000 & 20 & 59 & 107 & 131 & 123 & 109   & 1000 & 20 & 50 & 54 & 54 & 55 & 51 \\
% 		1000 & 50 & 48 & 94  & 114 & 106 & 99    & 1000 & 50 & 53 & 57 & 55 & 54 & 51 \\
% 		\hline
% 		10000 & 5  & 193 & 524 & 906 & $\times$ & $\times$   & 10000 & 5  & 142 & 232 & 298 & 370 & 408 \\
% 		10000 & 10 & 162 & 457 & 815 & $\times$ & $\times$   & 10000 & 10 & 121 & 180 & 261 & 320 & 328 \\
% %		10000 & 20 & 146 & 398 & 776 & $\times$ & $\times$   & 10000 & 20 & 101 & 158 & 236 & 284 & 300 \\
% 		10000 & 50 & 114 & 318 & 704 & 888      & $\times$   & 10000 & 50 & 87  & 148 & 224 & 261 & 278
% 	\end{tabu}
	\caption{Iteration counts for the heterogeneous, elliptic,
          indefinite problem (left) and for the convection--diffusion
          problem with zero-divergence convection coefficient
          \eqref{conv:zero-div} (right), varying the parameter
          $\kappa$ (left) and the constant $b$ (right), as well as
          $a_\text{max} > 1$ and the number of subdomains $N$ for fixed $h = 1/600$.}
	\label{Table:Heterogeneous_nglob600}
\end{table}

In Table~\ref{Table:Coarse_space_size_nglob600} we display the size of
the GenEO coarse space employed, along with comparison figures from
the homogeneous case (labelled $a_\text{max} = 1$). We note that, at
most, only a small number of additional eigenvectors are required in
the coarse space in order to treat the heterogeneity for any
$a_\text{max}$ used, thus showing robustness to contrasts in the
diffusion coefficient. We also see that the size of the coarse space
grows with $N$, however, the average number of eigenvectors per
subdomain decreases with $N$ so that we need to solve only small
eigenvalue problems for a small number of eigenvectors.

In conclusion, the GenEO method is well-equipped to deal with heterogeneities in the coefficient $A$, allowing us to treat the heterogeneous problem similarly to the homogeneous one.

\begin{table}[ht]
	\centering
	\tabulinesep=1.2mm
	%\footnotesize
	\begin{tabu}{c|ccccc}
		& \multicolumn{5}{c}{$N$} \\
		$a_\text{max}$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		1  & 212 (53.0) & 624 (39.0) & 1060 (29.4) & 1480 (23.1) & 1800 (18.0) \\
%		5  & 210 (52.5) & 615 (38.4) & 1050 (29.2) & 1455 (22.7) & 1814 (18.1) \\
		10 & 209 (52.3) & 613 (38.3) & 1046 (29.1) & 1447 (22.6) & 1828 (18.3) \\
%		20 & 205 (51.3) & 612 (38.3) & 1053 (29.3) & 1443 (22.5) & 1838 (18.4) \\
		50 & 202 (50.5) & 612 (38.3) & 1055 (29.3) & 1442 (22.5) & 1845 (18.5)
	\end{tabu}
	\caption{The size of the coarse space for the homogeneous
          problem (denoted $a_\text{max} = 1$) and the heterogeneous
          inclusions and channels problem, varying $a_\text{max}$ and
          the number of subdomains $N$ for fixed $h = 1/600$. The average number of eigenvectors per subdomain, namely the size of the coarse space divided by $N$, is given in parenthesis.}
	\label{Table:Coarse_space_size_nglob600}
\end{table}

\subsection{Dependence on mesh refinement}
\label{subsec:numerics-meshrefinement}

In this subsection we explore dependence upon the mesh spacing $h$. We consider problem  \eqref{eq:helmholtz}
with $A$ given as in \eqref{eq:hetcoeff} and we set  $\kappa = 1000$
and $a_\text{max} = 50$. Table~\ref{Table:Indefinite_heterogeneous_kappa1000_amax50} (left)
shows how the iteration count and the size of the coarse space vary with $h$. We
note that the iteration count remains stable as
$h$ decreases and the number $N$ of subdomains grows. On
the other hand, the size of the coarse space appears to
grow at a rate slightly slower than $\mathcal{O}(h^{-1})$ as $h$ is
decreased. This is in full agreement with similar results in
\cite[Table 1]{peter} for positive-definite problems in the case of minimal
overlap $\delta \sim h$.

As in \cite{peter}, we repeat our experiment for the case of
generous overlap $\delta \sim H$. We fix the subdomain size $H$ and
the overlap $\delta$ independent of $h$, in particular to that given
by minimal overlap on the coarsest mesh size $h=\frac1{200}$, such that $\delta
=\frac{1}{100}$. The partition of unity is chosen to vary smoothly
over the entire extent of the overlap. (For details of the implementation
within FreeFem, see \cite[Section 4.1]{jolivet:2012}.) The iteration counts presented
in Table~\ref{Table:Indefinite_heterogeneous_kappa1000_amax50} (right)
for this setup remain stable and are essentially identical to those for minimal overlap
in the left table, but in addition, we now also observe that the size of the coarse space
remains bounded as $h\rightarrow 0$, which is again in agreement with the
results in \cite[Table 1]{peter}.

In all cases, our results show  that the dimension of the coarse space depends on $N$,
and grows approximately as $\mathcal{O}(N^{2/3})$; this means the
number of eigenvectors chosen per subdomain decreases with $N$ at
approximately the rate $\mathcal{O}(N^{-1/3})$.

\begin{table}[t]
	\centering
	\tabulinesep=1.2mm
	\begin{tabu}{c|ccc|ccc}
		& \multicolumn{3}{c|}{$N$} & \multicolumn{3}{c}{$N$}\\
		$h$ & 16 & 36 & 100 & 16 & 36 & 100\\
		\hline
		$\frac{1}{200}$ & 87 (185) & 115 (318) & 90 (598) &
				87 (185) & 115 (318) & 90 (598) \\
		$\frac{1}{400}$ & 89 (419) & 107 (661) & 91 (1214) &
                88 (225) & 109 (356) & 94 (639) \\
		$\frac{1}{600}$ & 94 (612) & 114 (1055) & 99 (1845) &
                92 (227) & 116 (384) & 99 (672) \\
		$\frac{1}{800}$ & 95 (847) & 115 (1329) & 100 (2478) &
                93 (228) & 116 (379) & 100 (680) \\
	\end{tabu}
	% \begin{tabu}{c|ccccc|ccccc}
	% 	& \multicolumn{10}{c}{$N$} \\
	% 	$h$ & 4 & 16 & 36 & 64 & 100 & 4 & 16 & 36 & 64 & 100 \\
	% 	\hline
	% 	$\frac{1}{200}$ & 48 & 87 & 115 & 100 & 90    & 67  & 185 & 318  & 417  & 598  \\
	% 	$\frac{1}{400}$ & 47 & 91 & 110 & 101 & 93    & 119 & 354 & 589  & 814  & 1056 \\
	% 	$\frac{1}{600}$ & 50 & 97 & 119 & 110 & 101   & 164 & 492 & 840  & 1156 & 1451 \\
	% 	$\frac{1}{800}$ & 51 & 99 & 120 & 113 & 104   & 209 & 614 & 1001 & 1475 & 1887 \\
	% \end{tabu}
        %
	% \begin{tabu}{c|ccccc|ccccc}
	% 	& \multicolumn{10}{c}{$N$} \\
	% 	$h$ & 4 & 16 & 36 & 64 & 100 & 4 & 16 & 36 & 64 & 100 \\
	% 	\hline
	% 	$\frac{1}{200}$ & 48 & 87 & 115 & 100 & 90    & 67 & 185 & 318 & 417 & 598 \\
	% 	$\frac{1}{400}$ & 47 & 88 & 109 & 104 & 94    & 81 & 225 & 356 & 462 & 639 \\
	% 	$\frac{1}{600}$ & 49 & 92 & 116 & 112 & 99    & 83 & 227 & 384 & 469 & 672 \\
	% 	$\frac{1}{800}$ & 49 & 93 & 116 & 113 & 100   & 83 & 228 & 379 & 481 & 680 \\
	% \end{tabu}
	\caption{Iteration count and size of the coarse space (in brackets) for
          minimal overlap $\delta \sim h$ (left) and for generous
          overlap $\delta \sim H$ (right) for problem \eqref{eq:helmholtz}
          with heterogeneous $A$ as in \eqref{eq:hetcoeff}, varying $h$ and
          $N$ for $\kappa = 1000$ and $a_\text{max} = 50$ fixed.}
	\label{Table:Indefinite_heterogeneous_kappa1000_amax50}
\end{table}

\subsection{The effect of the convection field}
\label{subsec:numerics-convfield}

For problem \eqref{eq:convdiff} the specific form of $\mathbf{b}$  can play an  important role.
Here we consider some further examples to illustrate this point and show how the divergence of $\mathbf{b}$ can dictate performance, as predicted by the theory.
%
We start with the  homogeneous case $A = I$,  and with a circulating convection field. Here the problem is posed on $(-1,1)\times(0,1)$ and the convection coefficient is given as
\begin{align}
\label{conv:circulating}
\mathbf{b} = b \, (2y(1-x^2),-2x(1-y^2))^{T},
\end{align}
illustrated in Figure~\ref{fig:conv_circ}. Results varying $b$, which
controls the strength of the convective term, are given in Table
\ref{Table:Convection_circulating_homogeneous_nglob600} (left). As before,
GenEO  behaves robustly  for  $b$ up to at least $1000$.

\begin{figure}[t]
	\centering
	\subfigure[Without oscillations: $\mathbf{b}$ given by \eqref{conv:circulating}.\label{fig:conv_circ}]{\includegraphics[width=0.49\textwidth,trim=1.8cm 0cm 1.8cm 0cm ,clip]{convection_circulating}}
	\subfigure[With oscillations: $\mathbf{b}$ given by \eqref{conv:circulating-sine-radial} with $n=4$.\label{fig:conv_circ_osc}]{\includegraphics[width=0.49\textwidth,trim=1.8cm 0cm 1.8cm 0cm ,clip]{convection_circulating_oscillations}}
	\caption{Circulating convection fields with and without oscillation in the radial direction.}
	\label{fig:conv_fields_circ}
\end{figure}

\begin{table}[t]
	\centering
	\tabulinesep=1.2mm
	\begin{tabu}{c|ccccc}
		& \multicolumn{5}{c}{$N$} \\
		$b$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		1 & 18 & 18 & 18 & 18 & 18 \\
		10 & 24 & 24 & 22 & 21 & 20 \\
		100 & 43 & 44 & 41 & 36 & 33 \\
		1000 & 31 & 34 & 35 & 35 & 36 \\
		10000 & 143 & 231 & 282 & 314 & 339 \\
		\hline
		$-$ & 316 & 931 & 1584 & 2170 & 2796
	\end{tabu} \qquad\qquad
	% \begin{tabu}{c|ccccccccc}
	% 	& \multicolumn{9}{c}{$N$} \\
	% 	$b$ & 4 & 9 & 16 & 25 & 36 & 49 & 64 & 81 & 100 \\
	% 	\hline
	% 	1 & 18 & 17 & 18 & 17 & 18 & 18 & 18 & 18 & 18 \\
	% 	10 & 24 & 23 & 24 & 22 & 22 & 21 & 21 & 20 & 20 \\
	% 	100 & 43 & 45 & 44 & 42 & 41 & 36 & 36 & 33 & 33 \\
	% 	1000 & 31 & 28 & 34 & 31 & 35 & 34 & 35 & 35 & 36 \\
	% 	10000 & 143 & 208 & 231 & 254 & 282 & 263 & 314 & 291 & 339 \\
	% 	\hline\hline
	% 	$-$ & 316 & 620 & 931 & 1255 & 1584 & 1801 & 2170 & 2424 & 2796
	% \end{tabu}
	\begin{tabu}{c|ccccc}
		& \multicolumn{5}{c}{$N$} \\
		$n$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		1 & 30 & 33 & 35 & 35 & 36 \\
		2 & 35 & 44 & 49 & 45 & 49 \\
		4 & 44 & 64 & 65 & 57 & 57 \\
		8 & 46 & 66 & 70 & 65 & 60
	\end{tabu}
	\caption{Iteration counts for problem \eqref{eq:convdiff} with
          $A= I$ and  with circulating convection coefficient for
            $h = 1/600$. Left:  Using \eqref{conv:circulating} and
            varying the parameter $b$ and the number of subdomains
            $N$; the coarse space size (independent of $b$) is
            tabulated in the final row. Right: Using
            \eqref{conv:circulating-sine-radial} with radial
            oscillations and $b=1000$, varying the parameter $n$ and the
            number of subdomains $N$.}
	\label{Table:Convection_circulating_homogeneous_nglob600}
\end{table}

As well as varying the strength of the convective term, we can
also add local variation. To this end,  we  add sinusoidal
variation of increasing frequency in the radial direction
(perpendicular to the characteristics
of the convection field). That is, we consider
\begin{align}
\label{conv:circulating-sine-radial}
\mathbf{b} = b \, \sin( n\pi(1-x^2)(1-y^2) ) (2y(1-x^2),-2x(1-y^2))^{T},
\end{align}
for a parameter $n$; see Figure~\ref{fig:conv_circ_osc}. Note that for
any choice of $n$ this convection coefficient is divergence-free
since $\nabla \cdot \mathbf{b} = 0$. Thus, here we
illustrate the effect of local variation without changing the
divergence. Results for $b=1000$ and varying $n$ are given in Table
\ref{Table:Convection_circulating_homogeneous_nglob600} (right),
where we see that iteration counts slightly increase with the
frequency parameter $n$ but that this remains mild and the coarse
space continues to provide a robust preconditioner as $N$ increases.

We now explore the role the local variation of the divergence of
$\mathbf{b}$ plays by considering a simple unidirectional convection
field with sinusoidal variation added in such a way as to vary
$\nabla \cdot \mathbf{b}$. In particular, we consider
\begin{align}
\label{conv:unidirectional-oscillations}
\mathbf{b} = b \, (1+\sin(m\pi(2x+y))) (1+\sin(2\pi(2y-x))) (2,1)^{T},
\end{align}
see Figure~\ref{fig:conv_field_unidir}, on the unit square. In this
case, we also choose the heterogeneous diffusion coefficient $A$ in
\eqref{eq:hetcoeff} to incorporate the full range of heterogeneity.

Here $\mathbf{b}$ includes oscillation both
across characteristics and along characteristics. The term
$(1+\sin(2\pi(2y-x)))$ introduces oscillations that do not
change the strength of the divergence. On the
other hand, the term $(1+\sin(m\pi(2x+y)))$ introduces oscillations
along characteristics and as we increase their frequency through the
parameter $m$ we increase the strength of the divergence locally. This can be
seen visually in Figure~\ref{fig:conv_field_unidir} where we have
$m=4$ oscillations along any unit vector parallel to $(2,1)^{T}$ and
$2$ oscillations along any unit vector perpendicular to
$(2,1)^{T}$. To see how this affects performance we fix $b = 1000$ and
$a_\text{max} = 50$ and display results for increasing $m$ in Table
\ref{Table:Convection_unidirectional_oscillating_heterogeneous_nglob600}. This
time we see that increasing the oscillations has a significant impact
on the iteration counts and the GenEO coarse space starts to
struggle if  $m$ gets too big. This observation aligns with the
theory which suggests that a large divergence can hamper the
effectiveness of the coarse space.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth,trim=1.8cm 0cm 1.8cm 0cm ,clip]{convection_unidirectional_oscillations}
	\caption{Unidirectional convection field with oscillations: $\mathbf{b}$ given by \eqref{conv:unidirectional-oscillations} with $m=4$.}
    \label{fig:conv_field_unidir}
\end{figure}

\begin{table}[t]
	\centering
	\tabulinesep=1.2mm
	\begin{tabu}{c|ccccc}
		& \multicolumn{5}{c}{$N$} \\
		$m$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		0 & 53 & 57 & 55 & 54 & 51 \\
		2 & 56 & 85 & 88 & 95 & 78 \\
		4 & 50 & 97 & 143 & 162 & 123 \\
		8 & 56 & 79 & 171 & 133 & 181 \\
	\end{tabu}
	\caption{Iteration counts for the heterogeneous convection--diffusion problem with oscillating unidirectional convection coefficient \eqref{conv:unidirectional-oscillations}, varying the parameter $m$ (which controls the size of $\nabla \cdot \mathbf{b}$) and the number of subdomains $N$, with fixed $h = 1/600$, $b = 1000$ and $a_\text{max} = 50$.}
	\label{Table:Convection_unidirectional_oscillating_heterogeneous_nglob600}
\end{table}

To summarise, the GenEO coarse space is able to handle variations in the convection field to an extent. However, should $\nabla \cdot \mathbf{b}$ become too large then the approach can lose robustness.

\subsection{Time evolution for convection--diffusion problems}
\label{subsec:numerics-timestepping}

Finally, we also include one experiment on time evolution for
convection--diffusion problems. The
underlying time-dependent problem for $u(\mathbf{x},t)$ over the
time-interval $(0,T)$ is given by
\begin{subequations}
\label{eq:convdiff_timedependent}
\begin{align}
\frac{\partial u}{\partial t}-\mathrm{div}( A \nabla u) + \mathbf{b}\cdot\nabla u + \kappa u &= g & & \text{in } \Omega \times (0,T), \\
u &= 0 & & \text{on } \partial\Omega \times (0,T), \\
u &= u_0 & & \text{on } \Omega \times \left\lbrace 0 \right\rbrace.
\end{align}
\end{subequations}
Consider using an implicit scheme in time to yield a semi-discrete
problem. In particular, by way of example, we consider the backward
Euler scheme with time-step $\Delta t > 0$ and set (without loss of generality) $\kappa = 0$, yielding
\begin{subequations}
\label{eq:convdiff_semidiscrete}
\begin{align}
-\mathrm{div}( A \nabla u^{n}) + \mathbf{b}\cdot\nabla u^{n} + \frac{1}{\Delta t} u^{n} &= g^{n} + \frac{1}{\Delta t} u^{n-1} & & \text{in } \Omega, \\
u^{n} &= 0 & & \text{on } \partial\Omega,
\end{align}
\end{subequations}
where $u^{n}(\mathbf{x}) \approx u(\mathbf{x},n \Delta t)$ and $u^0 =
u_0$ with a similar convention for $g$. The canonical expression of the semi-discrete problem at each time-step takes the form
\begin{subequations}
\label{eq:convdiff_timestepping}
\begin{align}
-\mathrm{div}( A \nabla u) + \mathbf{b}\cdot\nabla u + \frac{1}{\Delta t} u &= f & & \text{in } \Omega, \\
u &= 0 & & \text{on } \partial\Omega,
\end{align}
\end{subequations}
for some $f$ and it is this generic problem we consider solving. Other implicit time-stepping schemes will lead to similar PDE problems at each time-step, so this investigation covers the general case.

Since $1/\Delta t > 0$, it could be put completely into the
coefficient  $c^+$, as defined in \eqref{eq:splitc}, and thus used in
the definition of the GenEO coarse space. However, to allow better efficiency in
the case of variable time-stepping it would be better to build a
preconditioner that is independent of  the time-step size. So  we suppose that
a `median time-step' $\Delta t_0$ is chosen and we perform the splitting \eqref{eq:splitc} with
$$ c^+ = 1/\Delta t_0 \quad \text{and} \quad c^{-} =  1/\Delta t  - 1/\Delta t_0. $$
With this choice, the GenEO preconditioner is built---once only,
before time-stepping takes place---incorporating the
$1/\Delta t_{0}$ term, i.e., using the bilinear form
\begin{align*}
a_{\Omega_{i}}(u,v) &= \int_{\Omega_{i}}\left(A\nabla u\cdot{\nabla v}\, + \frac{1}{\Delta t_{0}} u v\right) dx.
\end{align*}
We  study the utility of this choice
by varying parameters $\Delta t_0$ and $\Delta t$.

\begin{table}[t]
	\centering
	\tabulinesep=1.2mm
	\begin{tabu}{c|ccccc}
		 & \multicolumn{5}{c}{$N$} \\
		$\Delta t$ & 4 & 16 & 36 & 64 & 100 \\
		\hline
		1000 & 53/53/44  & 57/56/49  & 55/55/51 &
                54/54/51 & 51/51/49 \\
	        0.1 & 53/53/44 & 57/56/49 & 55/55/51 & 54/54/51 & 51/51/49 \\
		0.001 & 50/50/43  & 53/53/48 & 53/53/50 &
                52/52/50 & 50/50/48\\
	\end{tabu}
	\caption{Iteration counts with $\Delta
          t_{0} = 10$ (left), $0.1$ (middle), and $0.001$ (right) for
          one time-step \eqref{eq:convdiff_timestepping} of backward Euler applied
          to the time-dependent convection--diffusion
          problem with heterogeneous diffusion coefficient \eqref{eq:hetcoeff}
          and unidirectional convection coefficient
          \eqref{conv:zero-div}, varying the time-step
          $\Delta t$ and the number of subdomains $N$, for fixed $h =
          1/600$, $b = 1000$ and $a_\text{max} = 50$.}
	\label{Table:Convection_time-stepping_unidirectional_oscillating_m0n2_heterogeneous_nglob600}
\end{table}
We take $\Omega = (0,1)^2$, $A$ as in \eqref{eq:hetcoeff}, and consider the divergence-free convection coefficient \eqref{conv:zero-div}, fixing $b = 1000$ and $a_\text{max} = 50$.
Results are given in Table~\ref{Table:Convection_time-stepping_unidirectional_oscillating_m0n2_heterogeneous_nglob600}
where we see that the GenEO preconditioner is robust to changes in
both $\Delta t_0$ and $\Delta t$ (with either $\Delta t \le \Delta t_0 $ or $\Delta t > \Delta t_0 $), thus providing
an effective and efficient preconditioner for implicit time-stepping of
non-self adjoint or indefinite time-dependent problems.

\subsection{Alternative two-level preconditioners and GenEO-type coarse spaces}
\label{subsec:alternative-geneo}

The theory in this paper and the numerical results above are for the
classical, additive two-level Schwarz preconditioner with the
GenEO coarse space in \eqref{eq:2-19}. The underlying generalised
eigenproblem in \eqref{eq:2-18} is based on the self-adjoint and positive-definite
subproblem \eqref{eq:2-4}, which inevitably ceases to provide a robust
preconditioner when the indefiniteness or non-self-adjointness is very strong.

Especially for indefinite problems, such as
\eqref{eq:helmholtz}, the \emph{Restricted Additive Schwarz} (RAS)
preconditioner \cite{cai_sarkis}
along with a deflation approach to incorporate
the coarse space has previously been shown to lead  to
significantly lower iteration counts and better robustness with respect
to the indefiniteness \cite{bootland:2021:GCS,bootland:2021:ACS}.

For the remainder of this section we return to problem \eqref{eq:helmholtz},
and start by repeating the
experiments  reported in Table~\ref{Table:Heterogeneous_nglob600} (left),
but this time we use RAS instead of additive Schwarz for the one-level part of the preconditioner,
and we combine this with the coarse solve using a deflation approach. Otherwise the setup is identical to that in Table~\ref{Table:Heterogeneous_nglob600} (left). See, e.g., \cite{bootland:2021:GCS} for more details of this `RAS plus deflation' algorithm.
Results for this `RAS plus deflation' approach are given in Table
\ref{Table:RAS} (right) which can be compared with the corresponding  results from Table~\ref{Table:Heterogeneous_nglob600}  (given again here on the left for convenience). We see that the `RAS plus deflation' algorithm
requires roughly half the number of iterations needed by the standard algorithm,
but it does not yield any significantly improved
robustness with respect to the indefiniteness.
\begin{table}[t]
\centering
\tabulinesep=1.2mm
\begin{tabu}{cc|cccc|cccc}
	& & \multicolumn{8}{c}{$N$} \\
	$\kappa$ & $a_\text{max}$ & 16 & 36 & 64 & 100 & 16 & 36 & 64 & 100 \\
	\hline
	10 & 5 & 18 & 18 & 19 & 19     & 9 & 9 & 9 & 9 \\
	10 & 10 & 18 & 19 & 19 & 19      & 9 & 9 & 9 & 9 \\
%	10 & 20 & 18 & 18 & 19 & 19 & 19     & 9 & 9 & 9 & 9 \\
	10 & 50 & 18 & 20 & 19 & 19     & 9 & 9 & 9 & 9 \\
	\hline
	100 & 5 &  30 & 26 & 23 & 22     & 11 & 10 & 10 & 9 \\
	100 & 10 & 26 & 24 & 23 & 22     & 11 & 10 & 10 & 9 \\
%	100 & 20 & 24 & 23 & 22 & 21     & 10 & 10 & 10 & 10 \\
	100 & 50 & 22 & 22 & 20 & 20     & 9 & 9 & 9 & 9 \\
	\hline
	1000 & 5 & 140 & 177 & 167 & 138     & 62 & 76 & 70 & 57 \\
	1000 & 10 & 118 & 146 & 131 & 108     & 50 & 62 & 55 & 45 \\
%	1000 & 20 & 107 & 131 & 123 & 109    & 46 & 54 & 50 & 44 \\
	1000 & 50 & 94  & 114 & 106 & 99     & 38 & 46 & 43 & 39 \\
	\hline
	10000 & 5 & 524 & 906 & $\!\!1000+\!\!$ & $\!\!1000+\!\!$ &   297 & 504 & 628 & 753 \\
	10000 & 10 & 457 & 815 & $\!\!1000+\!\!$& $\!\!1000+\!\!$ &    234 & 445 & 548 & 644 \\
%	10000 & 20 & 398 & 776 & $\times$ & $\times$ &    197 & 409 & 505 & 582 \\
	10000 & 50 & 318 & 704 & 888      & $\!\!1000+\!\!$ &    171 & 372 & 464 & 538
\end{tabu}
\caption{Iteration counts for problem \eqref{eq:helmholtz} with
heterogeneous $A$ as in \eqref{eq:hetcoeff}, using the GenEO coarse space based on
\eqref{eq:2-18} and varying $\kappa$, $a_\text{max} > 1$ and $N$
with $h = 1/600$ fixed. Left: Classical two-level, additive Schwarz.
Right: Restricted additive Schwarz and deflation.}
\label{Table:RAS}
\end{table}

In \cite{bootland:2021:GCS} we also compared the GenEO coarse space
based on the eigenproblem \eqref{eq:2-18}, denoted $\Delta$-GenEO
in \cite{bootland:2021:GCS}, with an alternative approach first
introduced for the Helmholtz problem in~\cite{bootland:2021:ACS},
going under the name of $\mathcal{H}$-GenEO.
\begin{definition}\label{def:5-12}
($\mathcal{H}$-GenEO eigenproblem). For each $j=1,\ldots,N$, we define the following generalized eigenvalue problem
\begin{equation}\label{eq:5-12}
\text{Find} \quad (p, \lambda) \in {\tV}_j\backslash \{0\} \times \mathbb{R} \quad \text{such that} \quad      b_{\Omega_{j}}(p,v) = \lambda \,a_{\Omega_{j}}(\Xi_{j}(p), \Xi_{j}(v)),\quad {\rm for}\;\,{\rm all}\;\,v\in \widetilde{V}_{j},
\end{equation}
where $b_{\Omega_j}(\cdot,\cdot)$ is given in \eqref{eq:2-10} and $\Xi_{j}$ is the local partition of unity operator from Definition~\ref{def:2-0}.
\end{definition}

Recalling \eqref{eq:2-18},  we see that the key difference in $\mathcal{H}$-GenEO compared with $\Delta$-GenEO is the
use  of the bilinear form $b_{\Omega_j}(\cdot,\cdot)$ of the underlying
indefinite problem on the left-hand side. Note that this also implies that
the eigenvalues $\lambda$ in \eqref{eq:5-12} {can be negative}.
Thus,
when incorporating eigenvectors into the coarse space using the
threshold $\lambda < \lambda_\text{max}$ we also include all
negative eigenvalues (see again \cite{bootland:2021:GCS} for  details).

In our final set of results, Table~\ref{Table:H-GenEO}, we repeat the
experiments in Table~\ref{Table:RAS}
using the GenEO coarse space based on the $\mathcal{H}$-GenEO
eigenproblem in \eqref{eq:5-12}, again with an otherwise identical
setup. We see that for small $\kappa$ the iteration counts are almost
identical. For large $\kappa$, we see that $\mathcal{H}$-GenEO leads to
much lower iteration counts, such that GMRES
converges in less than $50$ iterations even for $\kappa = 10000$ when
using the `RAS plus deflation' approach. Unfortunately, a theoretical
justification for this excellent performance of the $\mathcal{H}$-GenEO
method is still lacking. We note that for larger $\kappa$ the coarse
space induced by the
$\mathcal{H}$-GenEO eigenproblem in \eqref{eq:5-12} is slightly larger
than that induced by the eigenproblem in \eqref{eq:2-18}
(see \cite[Table 2]{bootland:2021:GCS}). Nonetheless, this
increase is relatively modest compared to the
reduction in iteration counts that can be achieved.

\begin{table}[t]
\centering
\tabulinesep=1.2mm
\begin{tabu}{cc|cccc|cccc}
	& & \multicolumn{8}{c}{$N$} \\
	$\kappa$ & $a_\text{max}$ & 16 & 36 & 64 & 100 & 16 & 36 & 64 & 100 \\
	\hline
	10 & 5 & 18 & 18 & 19 & 19 & 9 & 9 & 9 & 9  \\
	10 & 10 & 18 & 19 & 19 & 19 & 9 & 9 & 9 & 9   \\
%	10 & 20 & 18 & 19 & 19 & 19 & 9 & 9 & 9 & 9   \\
	10 & 50 & 18 & 19 & 19 & 19 & 9 & 9 & 9 & 9    \\
	\hline
	100 & 5 & 18 & 19 & 19 & 19 & 9 & 9 & 9 & 9  \\
	100 & 10 & 18 & 19 & 19 & 19 & 9 & 9 & 9 & 9 \\
%	100 & 20 & 18 & 19 & 19 & 19 & 9 & 9 & 9 & 9   \\
	100 & 50 & 18 & 19 & 19 & 19 & 8 & 9 & 9 & 9  \\
	\hline
	1000 & 5 & 43 & 36 & 29 & 32 & 12 & 12 & 11 & 12  \\
	1000 & 10 & 36 & 43 & 23 & 24 & 11 & 11 & 10 & 10 \\
%	1000 & 20 & 32 & 53 & 26 & 29 & 14 & 12 & 12 & 13 \\
	1000 & 50 & 28 & 31 & 24 & 26 & 12 & 11 & 11 & 12  \\
	\hline
	10000 & 5 & 134 & 173 & 192 & 258 & 35 & 35 & 43 & 45   \\
	10000 & 10 & 113 & 147 & 191 & 192 & 21 & 29 & 41 & 34  \\
%	10000 & 20 & 92 & 125 & 168 & 197 & 23 & 25 & 41 & 31  \\
	10000 & 50 & 92 & 109 & 173 & 182 & 19 & 25 & 48 & 26
\end{tabu}
\caption{Iteration counts for problem \eqref{eq:helmholtz} with
  heterogeneous $A$ as
  in \eqref{eq:hetcoeff}, using the $\mathcal{H}$-GenEO coarse space based on
  \eqref{eq:5-12} and varying $\kappa$, $a_\text{max} > 1$ and $N$
  with $h = 1/600$ fixed. Left: Classical two-level, additive Schwarz.
  Right: Restricted additive Schwarz and deflation.}
\label{Table:H-GenEO}
\end{table}

These results provide an insight into the power of using generalised
eigenproblems to yield coarse spaces for challenging indefinite or
non-self-adjoint problems, which has yet to be fully explored even
numerically. A number of theoretical obstacles remain in order to analyse
the effect of such GenEO-type methods, but theory in this direction may
provide a greater understanding of where such approaches can be
successful and how to define appropriate, problem-dependent
generalised eigenproblems to incorporate the salient properties of the
underlying problem.
